Segment Any Anomaly without Training via Hybrid Prompt Regularization

We present a novel framework, i.e., Segment Any Anomaly + (SAA+), for zero-shot anomaly segmentation with hybrid prompt regularization to improve the adaptability of modern foundation models. Existing anomaly segmentation models typically rely on domain-specific fine-tuning, limiting their generalization across countless anomaly patterns. In this work, inspired by the great zero-shot generalization ability of foundation models like Segment Anything, we first explore their assembly to leverage diverse multi-modal prior knowledge for anomaly localization. For non-parameter foundation model adaptation to anomaly segmentation, we further introduce hybrid prompts derived from domain expert knowledge and target image context as regularization. Our proposed SAA+ model achieves state-of-the-art performance on several anomaly segmentation benchmarks, including VisA, MVTec-AD, MTD, and KSDD2, in the zero-shot setting. We will release the code at \href{https://github.com/caoyunkang/Segment-Any-Anomaly}{https://github.com/caoyunkang/Segment-Any-Anomaly}.

==> tables/ablation.tex <==
\begin{table}[t]
\centering
\caption{Ablation Study. Best scores are highlighted in \textbf{bold}. \cyk{tu be updated...}}
\label{tab:ablation}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{c|c|cc|cccc|cc|c} % @{}
\toprule
\multirow{2}{*}{} &
  \multirow{2}{*}{Prompt} &
  \multicolumn{1}{c|}{\multirow{2}{*}{Saliency}} &
  \multirow{2}{*}{Suppression} &
  \multicolumn{4}{c|}{Dataset} &
  \multicolumn{2}{c|}{Defect   Type} &
  \multirow{2}{*}{Total} \\ \cmidrule(lr){5-10}
 &
   &
  \multicolumn{1}{c|}{} &
   &
  \multicolumn{1}{c|}{VisA} &
  \multicolumn{1}{c|}{MVTec-AD} &
  \multicolumn{1}{c|}{KSDD2} &
  MTD &
  \multicolumn{1}{c|}{Texture} &
  Object &
   \\ \midrule
\multirow{12}{*}{$\mathcal{F}_{p}$} &
  \multirow{4}{*}{general} &
   &
   &
  \multicolumn{1}{c|}{13.59} &
  \multicolumn{1}{c|}{24.01} &
  \multicolumn{1}{c|}{4.27} &
  12.93 &
  \multicolumn{1}{c|}{18.34} &
  19.57 &
  18.64 \\ \cmidrule(l){5-11} 
 &
   &
   &
  \checkmark &
  \multicolumn{1}{c|}{22.36} &
  \multicolumn{1}{c|}{37.43} &
  \multicolumn{1}{c|}{{\ul \textit{59.41}}} &
  34.06 &
  \multicolumn{1}{c|}{24.71} &
  {\ul \textit{54.23}} &
  31.84 \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
   &
  \multicolumn{1}{c|}{18.39} &
  \multicolumn{1}{c|}{27.05} &
  \multicolumn{1}{c|}{12.45} &
  16.56 &
  \multicolumn{1}{c|}{21.29} &
  26.72 &
  22.60 \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
  \checkmark &
  \multicolumn{1}{c|}{{\ul \textit{25.78}}} &
  \multicolumn{1}{c|}{37.49} &
  \multicolumn{1}{c|}{\textbf{59.80}} &
  {\ul \textit{35.20}} &
  \multicolumn{1}{c|}{{\ul \textit{26.55}}} &
  \textbf{54.68} &
  {\ul \textit{33.34}} \\ \cmidrule(l){2-11} 
 &
  \multirow{4}{*}{manual} &
   &
   &
  \multicolumn{1}{c|}{12.30} &
  \multicolumn{1}{c|}{16.06} &
  \multicolumn{1}{c|}{0.76} &
  11.27 &
  \multicolumn{1}{c|}{16.25} &
  6.13 &
  13.81 \\ \cmidrule(l){5-11} 
 &
   &
   &
  \checkmark &
  \multicolumn{1}{c|}{19.73} &
  \multicolumn{1}{c|}{36.41} &
  \multicolumn{1}{c|}{51.35} &
  34.64 &
  \multicolumn{1}{c|}{23.68} &
  49.72 &
  29.96 \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
   &
  \multicolumn{1}{c|}{12.92} &
  \multicolumn{1}{c|}{18.93} &
  \multicolumn{1}{c|}{1.61} &
  14.88 &
  \multicolumn{1}{c|}{16.70} &
  12.56 &
  15.70 \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
  \checkmark &
  \multicolumn{1}{c|}{23.54} &
  \multicolumn{1}{c|}{36.72} &
  \multicolumn{1}{c|}{51.34} &
  34.81 &
  \multicolumn{1}{c|}{25.88} &
  50.01 &
  31.71 \\ \cmidrule(l){2-11} 
 &
  \multirow{4}{*}{mix} &
   &
   &
  \multicolumn{1}{c|}{15.70} &
  \multicolumn{1}{c|}{20.60} &
  \multicolumn{1}{c|}{1.49} &
  16.27 &
  \multicolumn{1}{c|}{18.92} &
  14.10 &
  17.76 \\ \cmidrule(l){5-11} 
 &
   &
   &
  \checkmark &
  \multicolumn{1}{c|}{19.39} &
  \multicolumn{1}{c|}{\textbf{39.47}} &
  \multicolumn{1}{c|}{58.55} &
  35.01 &
  \multicolumn{1}{c|}{24.72} &
  53.50 &
  31.66 \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
   &
  \multicolumn{1}{c|}{19.28} &
  \multicolumn{1}{c|}{24.43} &
  \multicolumn{1}{c|}{11.30} &
  14.58 &
  \multicolumn{1}{c|}{21.40} &
  21.83 &
  21.50 \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
  \checkmark &
  \multicolumn{1}{c|}{\textbf{27.07}} &
  \multicolumn{1}{c|}{{\ul \textit{39.40}}} &
  \multicolumn{1}{c|}{59.19} &
  \textbf{35.40} &
  \multicolumn{1}{c|}{\textbf{28.82}} &
  53.79 &
  \textbf{34.85} \\ \midrule
\multirow{12}{*}{$\mathcal{F}_{r}$} &
  \multirow{4}{*}{general} &
   &
   &
  \multicolumn{1}{c|}{6.27} &
  \multicolumn{1}{c|}{38.61} &
  \multicolumn{1}{c|}{12.44} &
  9.87 &
  \multicolumn{1}{c|}{17.67} &
  41.16 &
  23.34 \\ \cmidrule(l){5-11} 
 &
   &
   &
  \checkmark &
  \multicolumn{1}{c|}{{\ul \textit{14.95}}} &
  \multicolumn{1}{c|}{41.27} &
  \multicolumn{1}{c|}{37.94} &
  28.45 &
  \multicolumn{1}{c|}{22.97} &
  51.37 &
  29.82 \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
   &
  \multicolumn{1}{c|}{7.47} &
  \multicolumn{1}{c|}{37.57} &
  \multicolumn{1}{c|}{19.00} &
  15.04 &
  \multicolumn{1}{c|}{18.27} &
  40.77 &
  23.70 \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
  \checkmark &
  \multicolumn{1}{c|}{\textbf{15.92}} &
  \multicolumn{1}{c|}{42.10} &
  \multicolumn{1}{c|}{38.32} &
  27.58 &
  \multicolumn{1}{c|}{23.13} &
  54.21 &
  30.64 \\ \cmidrule(l){2-11} 
 &
  \multirow{4}{*}{manual} &
   &
   &
  \multicolumn{1}{c|}{6.74} &
  \multicolumn{1}{c|}{26.21} &
  \multicolumn{1}{c|}{9.98} &
  14.81 &
  \multicolumn{1}{c|}{15.05} &
  23.96 &
  17.20 \\ \cmidrule(l){5-11} 
 &
   &
   &
  \checkmark &
  \multicolumn{1}{c|}{13.36} &
  \multicolumn{1}{c|}{39.86} &
  \multicolumn{1}{c|}{{\ul \textit{45.03}}} &
  26.60 &
  \multicolumn{1}{c|}{19.60} &
  56.96 &
  28.61 \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
   &
  \multicolumn{1}{c|}{7.35} &
  \multicolumn{1}{c|}{27.01} &
  \multicolumn{1}{c|}{10.48} &
  15.69 &
  \multicolumn{1}{c|}{14.87} &
  27.49 &
  17.91 \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
  \checkmark &
  \multicolumn{1}{c|}{14.68} &
  \multicolumn{1}{c|}{\textbf{38.87}} &
  \multicolumn{1}{c|}{\textbf{46.76}} &
  26.90 &
  \multicolumn{1}{c|}{20.28} &
  55.26 &
  28.72 \\ \cmidrule(l){2-11} 
 &
  \multirow{4}{*}{mix} &
   &
   &
  \multicolumn{1}{c|}{6.32} &
  \multicolumn{1}{c|}{36.76} &
  \multicolumn{1}{c|}{7.66} &
  13.59 &
  \multicolumn{1}{c|}{20.61} &
  27.86 &
  22.36 \\ \cmidrule(l){5-11} 
 &
   &
   &
  \checkmark &
  \multicolumn{1}{c|}{12.82} &
  \multicolumn{1}{c|}{{\ul \textit{48.52}}} &
  \multicolumn{1}{c|}{39.35} &
  {\ul \textit{29.27}} &
  \multicolumn{1}{c|}{{\ul \textit{24.35}}} &
  {\ul \textit{59.21}} &
  {\ul \textit{32.77}} \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
   &
  \multicolumn{1}{c|}{7.46} &
  \multicolumn{1}{c|}{38.20} &
  \multicolumn{1}{c|}{18.48} &
  18.38 &
  \multicolumn{1}{c|}{20.99} &
  33.94 &
  24.11 \\ \cmidrule(l){5-11} 
 &
   &
  \checkmark &
  \checkmark &
  \multicolumn{1}{c|}{14.46} &
  \multicolumn{1}{c|}{\textbf{49.67}} &
  \multicolumn{1}{c|}{39.34} &
  \textbf{30.27} &
  \multicolumn{1}{c|}{\textbf{25.70}} &
  \textbf{60.40} &
  \textbf{34.07} \\ \bottomrule
\end{tabular}
}
\end{table}
